Homomorphism reconfiguration via homotopy

We consider the following problem for a fixed graph H: given a graph G and two H-colorings of G, i.e. homomorphisms from G to H, can one be transformed (reconfigured) into the other by changing one color at a time, maintaining an H-coloring throughout. This is the same as finding a path in the Hom(G,H) complex. For H=K_k this is the problem of finding paths between k-colorings, which was shown to be in P for k<=3 and PSPACE-complete otherwise by Cereceda et al. 2011. We generalize the positive side of this dichotomy by providing an algorithm that solves the problem in polynomial time for any H with no C_4 subgraph. This gives a large class of constraints for which finding solutions to the Constraint Satisfaction Problem is NP-complete, but finding paths in the solution space is P. The algorithm uses a characterization of possible reconfiguration sequences (paths in Hom(G,H)), whose main part is a purely topological condition described in algebraic terms of the fundamental groupoid of H seen as a topological space.

==> figureDefs.tex <==
\usepackage{tikz}
\usetikzlibrary{shapes,backgrounds,plothandlers,plotmarks,calc,arrows,fadings,patterns,decorations.pathmorphing}

\makeatletter
\pgfdeclarepatternformonly[\LineSpace,\LineWidth]{my horizontal lines}%
    {\pgfpointorigin}{\pgfqpoint{100pt}{1pt}}{\pgfqpoint{100pt}{\LineSpace}}%
    {
        \pgfsetcolor{\tikz@pattern@color}
        \pgfsetlinewidth{\LineWidth}
        \pgfpathmoveto{\pgfqpoint{0pt}{0.5pt}}
        \pgfpathlineto{\pgfqpoint{100pt}{0.5pt}}
        \pgfusepath{stroke}
    }
 
\pgfdeclarepatternformonly[\LineSpace,\LineWidth]{my vertical lines}%
    {\pgfpointorigin}{\pgfqpoint{1pt}{100pt}}{\pgfqpoint{\LineSpace}{100pt}}%
    {
        \pgfsetcolor{\tikz@pattern@color}
        \pgfsetlinewidth{\LineWidth}
        \pgfpathmoveto{\pgfqpoint{0.5pt}{0pt}}
        \pgfpathlineto{\pgfqpoint{0.5pt}{100pt}}
        \pgfusepath{stroke}
    } 
 
\pgfdeclarepatternformonly[\LineSpace,\LineWidth]{my grid}%
    {\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{\LineSpace}{\LineSpace}}
    {\pgfqpoint{\LineSpace}{\LineSpace}}%
    {
        \pgfsetcolor{\tikz@pattern@color}
        \pgfsetlinewidth{\LineWidth}
        \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
        \pgfpathlineto{\pgfqpoint{0pt}{\LineSpace + 0.1pt}}
        \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
        \pgfpathlineto{\pgfqpoint{\LineSpace + 0.1pt}{0pt}}
        \pgfusepath{stroke}
    }
 
\pgfdeclarepatternformonly[\LineSpace,\LineWidth]{my north east lines}
    {\pgfqpoint{-\LineWidth}{-\LineWidth}}{\pgfqpoint{\LineSpace}{\LineSpace}}
    {\pgfqpoint{\LineSpace}{\LineSpace}}%
    {
        \pgfsetcolor{\tikz@pattern@color}
        \pgfsetlinewidth{\LineWidth}
        \pgfpathmoveto{\pgfqpoint{-\LineWidth}{-\LineWidth}}
        \pgfpathlineto{\pgfqpoint{\LineSpace + 0.1pt}{\LineSpace + 0.1pt}}
        \pgfusepath{stroke}
    }
 
\pgfdeclarepatternformonly[\LineSpace,\LineWidth]{my north west lines}
    {\pgfqpoint{-\LineWidth}{-\LineWidth}}{\pgfqpoint{\LineSpace}{\LineSpace}}
    {\pgfqpoint{\LineSpace}{\LineSpace}}%
    {
        \pgfsetcolor{\tikz@pattern@color}
        \pgfsetlinewidth{\LineWidth}
        \pgfpathmoveto{\pgfqpoint{-\LineWidth}{\LineSpace}}
        \pgfpathlineto{\pgfqpoint{\LineSpace + 0.1pt}{-\LineWidth}}
        \pgfusepath{stroke}
    }
 
\pgfdeclarepatternformonly[\LineSpace,\LineWidth]{my crosshatch}%
    {\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{\LineSpace}{\LineSpace}}
    {\pgfqpoint{\LineSpace}{\LineSpace}}%
    {
        \pgfsetcolor{\tikz@pattern@color}
        \pgfsetlinewidth{\LineWidth}
        \pgfpathmoveto{\pgfqpoint{\LineSpace + 0.1pt}{0pt}}
        \pgfpathlineto{\pgfqpoint{0pt}{\LineSpace + 0.1pt}}
        \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
        \pgfpathlineto{\pgfqpoint{\LineSpace + 0.1pt}{\LineSpace + 0.1pt}}
        \pgfusepath{stroke}
    }
 
%\pgfdeclarepatternformonly[\LineSpace,\LineWidth]{my dots}%
%    {\pgfqpoint{-\LineSpace*0.25}{-\LineSpace*0.25}}
%    {\pgfqpoint{\LineSpace*0.25}{\LineSpace*0.25}}
%    {\pgfqpoint{\LineSpace*0.75}{\LineSpace*0.75}}%
%    {
%        \pgfsetcolor{\tikz@pattern@color}
%        \pgfpathcircle{\pgfqpoint{0pt}{0pt}}{\LineWidth}
%        \pgfusepath{fill}
%    }
\pgfdeclarepatternformonly[\LineSpace,\LineWidth]{my dots}%
    {\pgfpointorigin}
    {\pgfpoint{\LineSpace}{\LineSpace*0.866025*2}}
    {\pgfpoint{\LineSpace}{\LineSpace*0.866025*2}}%
    {
        \pgfsetcolor{\tikz@pattern@color}
        \pgfpathcircle{\pgfpoint{\LineSpace*0.25}{\LineSpace*0.866025*0.5}}{\LineWidth}
        \pgfpathcircle{\pgfpoint{\LineSpace*0.75}{\LineSpace*0.866025*1.5}}{\LineWidth}        
        \pgfusepath{fill}
    }
\makeatother
 
\newdimen\LineSpace
\newdimen\LineWidth
\tikzset{
    pattern space/.code={\LineSpace=#1},
    pattern space=3pt,
    pattern width/.code={\LineWidth=#1},
    pattern width=.4pt
}



\definecolor{cdred}{RGB}{200,20,20}
\definecolor{cdgreen}{RGB}{220,255,200}	
\definecolor{cdblue}{RGB}{130,145,255}	
\tikzset{ %
	dred/.style={pattern=my north west lines,pattern width=.6pt,pattern space=2.3pt,pattern color=red},
	dgreen/.style={pattern=my grid,pattern width=0.8pt,pattern space=2pt,pattern color=green!80!black},
	dblue/.style={pattern=my dots,pattern width=0.7pt,pattern space=2.3pt,pattern color=blue},	
	H/.style={circle,fill=gray!20,draw=gray!20,line width=2pt,inner sep=0pt,minimum size=15pt},
	He/.style={draw=gray!20,line width=12pt},
	G/.style={circle,fill=black,inner sep=0pt,minimum size=3pt},
	G1/.style={G,minimum size=5pt},
	Ge/.style={draw=black},
	v/.style={circle,draw=black!75,inner sep=0pt,minimum size=8pt},
	v1/.style={v,line width=1.5pt},
	Gv/.style={inner sep=0pt},
	Gve/.style={Ge,dashed},
}






\newcommand{\dfivegraph}{
		\node[H] (ha0) at (0:1.3) {};
		\node[H] (ha1) at (72:1.3) {};
		\node[H] (ha2) at (144:1.3) {};
		\node[H] (ha3) at (-144:1.3) {};		
		\node[H] (ha4) at (-72:1.3) {};	
		\draw[He]
			(ha0.center)--(ha1.center)
			(ha1.center)--(ha2.center)
			(ha2.center)--(ha3.center)
			(ha3.center)--(ha4.center)
			(ha4.center)--(ha0.center);
}

\newcommand{\dtengraph}{
	\begin{scope}[shift={(-1.3,0)}]		
		\node[H] (ha0) at (0:1.3) {};
		\node[H] (ha1) at (72:1.3) {};
		\node[H] (ha2) at (144:1.3) {};
		\node[H] (ha3) at (-144:1.3) {};		
		\node[H] (ha4) at (-72:1.3) {};	
		\draw[He]
			(ha0.center)--(ha1.center)
			(ha1.center)--(ha2.center)
			(ha2.center)--(ha3.center)
			(ha3.center)--(ha4.center)
			(ha4.center)--(ha0.center);
	\end{scope}	
	\begin{scope}[shift={(2.6,0)}]		
		\node[H] (hb0) at (180+0:1.3) {};
		\node[H] (hb1) at (180+72:1.3) {};
		\node[H] (hb2) at (180+144:1.3) {};
		\node[H] (hb3) at (180+-144:1.3) {};		
		\node[H] (hb4) at (180+-72:1.3) {};	
		\draw[He]
			(hb0.center)--(hb1.center)
			(hb1.center)--(hb2.center)
			(hb2.center)--(hb3.center)
			(hb3.center)--(hb4.center)
			(hb4.center)--(hb0.center);
	\end{scope}		
	\draw[He] (ha0.center)--(hb0.center);
}
\newcommand{\dtengraphflipped}{
	\begin{scope}[yscale=-1]
		\dtengraph;
	\end{scope}
}

\newcommand{\dtenprimgraph}{
	\begin{scope}[shift={(-2.7,0)}]		
		\node[H] (ha0) at (10:2) {};
		\node[H] (ha1) at (0:1) {};
		\node[H] (ha2) at (120:1) {};
		\node[H] (ha3) at (-120:1) {};
		\draw[He]
			(ha0.center)--(ha1.center)
			(ha1.center)--(ha2.center)
			(ha2.center)--(ha3.center)
			(ha3.center)--(ha1.center);
	\end{scope}	
	\begin{scope}[shift={(+2.7,0)},xscale=-1,yscale=-1]		
		\node[H] (hb0) at (10:2) {};
		\node[H] (hb1) at (0:1) {};
		\node[H] (hb2) at (120:1) {};
		\node[H] (hb3) at (-120:1) {};
		\draw[He]
			(hb0.center)--(hb1.center)
			(hb1.center)--(hb2.center)
			(hb2.center)--(hb3.center)
			(hb3.center)--(hb1.center);
	\end{scope}				
	\draw [He] (ha0.center)--(hb0.center);
}

\newcommand{\dninegraph}{
	\begin{scope}
		\node[H] (ha0) at (0:1) {};
		\node[H] (ha1) at (60:1) {};
		\node[H] (ha2) at (120:1) {};
		\node[H] (ha3) at (180:1) {};				
		\node[H] (ha4) at (-120:1) {};
		\node[H] (ha5) at (-60:1) {};
		\draw [He]
			(ha0.center)--(ha1.center)
			(ha1.center)--(ha2.center)
			(ha2.center)--(ha3.center)
			(ha3.center)--(ha4.center)
			(ha4.center)--(ha5.center)
			(ha5.center)--(ha0.center);						
	\end{scope}
	\begin{scope}[shift={(3,0)}]
		\node[H] (hb0) at (-180:1) {};
		\node[H] (hb1) at (60:1) {};
		\node[H] (hb2) at (-60:1) {};	
		\draw[He]
			(hb0.center)--(hb1.center)
			(hb1.center)--(hb2.center)
			(hb2.center)--(hb0.center);
	\end{scope}
	\draw[He] (ha0.center)--(hb0.center);
}
